Safe and Efficient Remote Application Code Execution on Disaggregated NVM Storage with eBPF

With rapid improvements in NVM storage devices, the performance bottleneck is gradually shifting to the network, thus giving rise to the notion of "data movement wall". To reduce the amount of data movement over the network, researchers have proposed near-data computing by shipping operations and compute-extensions closer to storage devices. However, running arbitrary, user-provided extensions in a shared, disaggregated storage environment presents multiple challenges regarding safety, isolation, and performance. Instead of approaching this problem from scratch, in this work we make a case for leveraging the Linux kernel eBPF framework to program disaggregated NVM storage devices. eBPF offers a safe, verifiable, and high-performance way of executing untrusted, user-defined code in a shared runtime. In this paper, we describe our experiences building a first prototype that supports remote operations on storage using eBPF, discuss the limitations of our approach, and directions for addressing them.

==> Makefile <==
.PHONY: all clean paper

all:  \
    tikz/storage-traditional.pdf \
    tikz/storage-disaggregated.pdf \
    tikz/storage-disaggregated-ops.pdf \
    tikz/ebpf-data.pdf \
    paper \
    ms

tikz/%.pdf: tikz/%.tex
	xelatex -output-directory=tikz/ $<
	pdfcrop $@

paper:
	latex-mk --pdflatex paper.tex || true

ms:
	latex-mk --pdflatex ms.tex || true
clean:
	rm -f paper.pdf paper-copy.pdf paper.bbl paper.blg paper.log paper.out paper.aux
	rm -f ms.pdf ms-copy.pdf ms.bbl ms.blg ms.log ms.out ms.aux

